The DEVIL is in the Details: A Diagnostic Evaluation Benchmark for Video Inpainting

Quantitative evaluation has increased dramatically among recent video inpainting work, but the video and mask content used to gauge performance has received relatively little attention. Although attributes such as camera and background scene motion inherently change the difficulty of the task and affect methods differently, existing evaluation schemes fail to control for them, thereby providing minimal insight into inpainting failure modes. To address this gap, we propose the Diagnostic Evaluation of Video Inpainting on Landscapes (DEVIL) benchmark, which consists of two contributions: (i) a novel dataset of videos and masks labeled according to several key inpainting failure modes, and (ii) an evaluation scheme that samples slices of the dataset characterized by a fixed content attribute, and scores performance on each slice according to reconstruction, realism, and temporal consistency quality. By revealing systematic changes in performance induced by particular characteristics of the input content, our challenging benchmark enables more insightful analysis into video inpainting methods and serves as an invaluable diagnostic tool for the field. Our code and data are available at https://github.com/MichiganCOG/devil .

==> input_abstract_blind.tex <==
\begin{abstract}
   Quantitative evaluation has increased dramatically among recent video inpainting work, but the video and mask content used to gauge performance has received relatively little attention.
   Although attributes such as camera and background scene motion inherently change the difficulty of the task and affect methods differently, existing evaluation schemes fail to control for them quantitatively, thereby providing little insight into inpainting failure modes.
   To address this gap, we propose the Diagnostic Evaluation of Video Inpainting on Landscapes (DEVIL) benchmark, which consists of two contributions: (i) a novel dataset of videos and masks labeled according to several key inpainting failure modes, and (ii) an evaluation scheme that samples slices of the dataset characterized by a fixed content attribute, and scores performance on each slice according to reconstruction, realism, and temporal consistency quality.
   By quantifying changes in performance induced by particular characteristics of the input content, our challenging benchmark enables insightful, comparative analysis into video inpainting methods and serves as an invaluable diagnostic tool for the field.
\end{abstract}


==> input_body_blind.tex <==
\section{Introduction}

\begin{figure*}
  \includegraphics[width=\linewidth]{figs/dataset-overview/dataset-overview}
  \caption{A visual overview of our DEVIL dataset. (a) The content attributes that characterize our dataset and are used to create dataset slices for evaluation (\ie, sets of video-mask pairs with a fixed attribute). We label low/high background scene motion or camera motion for videos exhibiting these attribute settings beyond a certain threshold (Section~\ref{sec:annotating-devil-source-video}). For occlusion masks, we construct sampling parameters that capture the desired attribute settings and use them to render masks (Section~\ref{sec:devil-masks-attributes}). (b) Videos, masks, and annotations from our dataset. A given video or mask may have multiple attribute labels or none; labels for the same attribute are mutually exclusive (\eg, a mask cannot have both low and high FG displacement).}
  \label{fig:dataset-overview}
\end{figure*}

Video inpainting, \ie, the task of filling in missing pixels in a video with plausible values, pushes the boundaries of modern video manipulation techniques and enables remarkable applications for film and social media such as watermark and foreground object removal~\cite{yeager_everything_2019,noauthor_production_2018}.
Compared to image inpainting, video inpainting is more challenging due to the additional temporal dimension, which not only increases the complexity of the solution space, but also places additional constraints on what constitutes a high-quality prediction, \ie, coherence in both spatial structure \textit{and} motion. Despite the difficulty of the task, modern results have become quite compelling thanks to the increasing amount of attention that the problem has received as of late~\cite{wang_video_2019,kim_deep_2019,xu_deep_2019,chang_free-form_2019,oh_onion-peel_2019,zhang_internal_2019,zeng_learning_2020,gao_flow-edge_2020}.

Quantitative evaluation has increased dramatically among recent video inpainting work; however, existing evaluation schemes underemphasize the importance of the contents of the videos and masks used to gauge performance.
Typically, video inpainting is evaluated as a reconstruction problem: performance is quantified by masking out arbitrary regions from the video (\ie, ``corrupting'' it) and scoring the model's ability to recover the masked-out values~\cite{xu_deep_2019,chang_free-form_2019,lee_copy-and-paste_2019}.
However, the difficulty of reconstruction depends on the mask's shape and motion, as well as the content present in the ``uncorrupted'' video.
For example, given a static mask, it is harder to inpaint a video captured by a fixed camera than one captured by a moving camera.
In the former case, the region beneath the mask is never visible, so the model effectively needs to ``hallucinate'' its appearance; in the latter case, the model could transfer appearance information from other frames, a strategy that lies at the heart of many video inpainting approaches~\cite{wexler_space-time_2007,huang_temporally_2016,lee_copy-and-paste_2019,oh_onion-peel_2019}.

\textit{The difficulty of video inpainting is inherently tied to the content of the videos and masks being inpainted;} with this principle in mind, we push for more emphasis on diagnostic evaluation that is quantitative and content-informed.
Such an approach would improve ablative analysis and enable concrete comparisons between modern inpainting methods under challenging conditions.
To date, the videos used for evaluation have been underappreciated in this regard, having been sourced from datasets for other tasks (\eg, facial analysis~\cite{shen_first_2015,rossler_faceforensics_2018} and object localization~\cite{perazzi_benchmark_2016,xu_youtube-vos_2018}) rather than selected to represent important \textit{inpainting} scenarios.
In particular, they contain biases that are essential for the original task, but hinder fine-grained analysis for video inpainting.
For example, object localization videos feature prominent, moving foreground objects; as a result, standard inpainting evaluation schemes underrepresent performance on foreground-free videos, which are targeted by the primary inpainting application of object removal~\cite{zhang_internal_2019}.
Furthermore, other types of motion, \eg, camera and background scene motion, noticeably impact video inpainting performance, but are not controlled for in standard datasets.

In this work, we propose the Diagnostic Evaluation of Video Inpainting on Landscapes (DEVIL) benchmark.
It is composed of two parts---the DEVIL dataset and the DEVIL evaluation scheme---which combine to enable a finer-grained analysis than has been possible in prior work.
Such granularity is achieved through \textit{content attributes}, \ie, properties of source videos or masks that characterize key failure modes by affecting how easily video inpainting models can borrow appearance information from nearby frames.
Specifically, the DEVIL dataset contains source videos labeled with low/high camera and background scene motion attributes, and occlusion masks labeled with low/high foreground displacement, pose motion, and size attributes (Figure~\ref{fig:dataset-overview}).
Meanwhile, the DEVIL evaluation scheme constructs several \textit{slices} of the DEVIL dataset---sets of video-mask pairs in which exactly one content attribute is kept fixed---and summarizes inpainting quality through metrics that capture reconstruction performance, realism, and temporal consistency (Section~\ref{sec:evaluation-metrics}).
By controlling for content attributes and summarizing inpainting quality per attribute across several metrics, our benchmark pinpoints the influence of challenging input data on the output in a way that is quantified, interpretable, and comparable across methods.

We use our benchmark to analyze the strengths and weaknesses of seven state-of-the-art video inpainting methods.
By quantifying their inpainting quality on ten DEVIL dataset slices under five evaluation metrics, we provide the most comprehensive and fine-grained evaluation of modern video inpainting methods to our knowledge.
Our head-to-head, multi-faceted comparisons allow us to draw several important conclusions.
For example, we show that video inpainting methods in which time and optical flow are carefully modeled consistently achieve the best performance across several types of input data.
We also show that the relative rankings between methods are highly sensitive to metrics as well as source video and mask content, illustrating that our benchmark fosters competition.
Finally, we show that controlling for source video and mask attributes reveals insightful failure modes which can be rapidly traced back to the design of the method in question.

Our comprehensive, diagnostic benchmark enables insightful analysis and serves as an invaluable tool for video inpainting research. To summarize, we provide the following contributions:
%
\begin{itemize}
  \item We present the first diagnostic dataset specifically designed for video inpainting to our knowledge, which includes annotations for content-based attributes that represent numerous inpainting failure modes;
  \item We introduce a comprehensive evaluation scheme that spans ten dataset slices and five evaluation metrics of video inpainting quality;
  \item We analyze seven state-of-the-art algorithms on our benchmark, providing the most comprehensive quantitative evaluation of video inpainting methods to date; and
  \item We identify systematic errors among video inpainting methods and highlight directions for future work.
\end{itemize}

\section{Related Work}

\subsection{Methods}
\label{sec:methods}

Most video inpainting algorithms borrow visual appearance information from known parts of the video to fill in unknown parts. For example, \textit{alignment-based methods} compute local or global alignments between neighboring frames, and then propagate pixels across aligned locations (alignments are found either through classical feature correspondences~\cite{granados_background_2012,ebdelli_video_2015} or deep neural networks~\cite{lee_copy-and-paste_2019,oh_onion-peel_2019,zeng_learning_2020}). \textit{Patch-borrowing methods} view videos as spatiotemporal tensors and iteratively paste cuboids or voxels from the known region into the unknown region to maximize global coherence~\cite{wexler_space-time_2007,granados_how_2012,newson_video_2014}. \textit{Flow-guided methods} propagate visual information along the optical flows estimated between consecutive frames, where the flow for unknown regions is computed iteratively or hierarchically based on known regions to improve performance~\cite{huang_temporally_2016,kim_deep_2019,xu_deep_2019,gao_flow-edge_2020}.

Although explicit appearance-borrowing is not leveraged for some methods, \eg, \textit{autoencoder-based methods}~\cite{wang_video_2019,chang_free-form_2019,chang_learnable_2019,zhang_internal_2019}, we use its prevalence to guide our experimental design. Specifically, we control for content-based attributes that affect the difficulty of borrowing relevant appearance information from other frames, which is possible through our varied data and comprehensive annotations.

\subsection{Datasets}
\label{sec:datasets}

The source video datasets used in early video inpainting work were small and oriented around qualitative analysis~\cite{wexler_space-time_2007,granados_how_2012,newson_video_2014}; as a result, it was difficult to compare the performance of early methods across a wide variety of scenarios. Recent work has instead used large-scale datasets---ranging in structure from aligned face videos~\cite{rossler_faceforensics_2018} and driving videos~\cite{dollar_pedestrian_2012} to unconstrained videos from the Internet~\cite{perazzi_benchmark_2016,xu_youtube-vos_2018}---to enable more comprehensive analysis. The foreground object segmentation datasets DAVIS~\cite{perazzi_benchmark_2016} and YouTube-VOS~\cite{xu_youtube-vos_2018} are often used since their annotations can be used for object removal; however, the ground truth in these applications is often ambiguous, especially for videos in which parts of the background are never visible.

In this work, we collect novel videos specifically for the inpainting task, emphasizing attributes that affect how well video inpainting models can transfer appearance information across frames. We also use videos of background scenes instead of videos with foreground objects, similar to Zhang \etal~\cite{zhang_internal_2019}. Unlike pre-existing datasets such as DAVIS and YouTube-VOS, ours provides ground truth for object removal applications and also allows us to isolate failure modes that are unrelated to foreground motion.

In terms of occlusion masks, static rectangles~\cite{xu_deep_2019,wang_video_2019} or foreground masks from other videos~\cite{kim_deep_2019,lee_copy-and-paste_2019,oh_onion-peel_2019,zhang_internal_2019} are commonly used. Procedural generation has also been explored as a way to generate masks that behave like real objects on a larger scale. For instance, Chang \etal~\cite{chang_learnable_2019,chang_free-form_2019} render several strokes on a canvas, where each stroke has several control points that randomly move with a certain probability. We extend their work by adding physical constraints for finer control over mask size and motion. We also choose our mask sampling parameters based on attributes that directly influence how easily video inpainting models can transfer appearance information across frames.

\section{Overview of the DEVIL Benchmark}

Before introducing the DEVIL benchmark for video inpainting, we first define the task itself. Let $V \in \{0, \dots, 255\}^{H \times W \times 3 \times T}$ be an input RGB video with $T$ frames and a resolution of $W \times H$. $V$ contains a placeholder value for missing voxels (\eg, 0) whose locations are indicated by an input occlusion mask $M \in \{0, 1\}^{H \times W \times T}$.
Video inpainting aims to produce an inpainted version of $V$, denoted $V^*$, with the following characteristics:
%
\begin{itemize}
  \item \textbf{Reconstruction performance:} $V^*$ is a faithful reconstruction of $V^{\textrm{gt}}$ in the scenario where $V$ is a ``corrupted'' video derived from some uncorrupted ground truth source video $V^{\textrm{gt}}$.
  \item \textbf{Realism:} $V^*$ is indistinguishable from a real video.
  \item \textbf{Temporal consistency:} $V^*$ exhibits minimal temporal flickering artifacts.
\end{itemize}
%
These criteria are defined more rigorously in Section~\ref{sec:evaluation-metrics}.

Our DEVIL benchmark is a collection of tools designed to provide a detailed understanding of video inpainting methods and their behavior across a variety of input data. There are two major components of our benchmark: (i) the DEVIL dataset, which contains source videos and occlusion masks that have been specially curated, rendered, and annotated to identify specific failure modes in video inpainting; and (ii) the DEVIL evaluation scheme, which reports a set of quality-based metrics on several ``slices'' of the DEVIL dataset, each of which represents a particular failure mode.

The DEVIL dataset captures content complexity along five video-level \textit{content attributes}, \ie, properties that affect the difficulty of inpainting a given video-mask pair by influencing the relevance and availability of appearance information from nearby frames. Specifically, it contains source videos with low and high camera and background (BG) scene motion, and occlusion masks with low and high foreground (FG) displacement, pose motion, and size (Figure~\ref{fig:dataset-overview}a).\footnote{The term ``foreground'' (FG) comes from FG object removal applications.} Furthermore, videos and masks are annotated with these attributes and their settings (low or high) to enable targeted evaluation that controls for their presence. Section~\ref{sec:devil-dataset} rigorously defines these attributes and describes our process for collecting videos, masks, and attribute annotations.

Meanwhile, our DEVIL evaluation scheme gauges inpainting quality under multiple \textit{slices} of our dataset, \ie, sets of video-mask pairs characterized by a certain attribute setting. Within each slice, exactly one dataset attribute is kept fixed while the others change freely. By measuring inpainting quality across several slices and metrics, DEVIL methodically quantifies the impact of major inpainting failure modes. In Section~\ref{sec:devil-evaluation}, we describe our DEVIL dataset slices and evaluation metrics in further detail.

\section{The DEVIL Dataset}
\label{sec:devil-dataset}

\subsection{Collecting Source Videos for the DEVIL}
\label{sec:collecting-source-videos-devil}

There is great value in evaluating inpainting methods on background scenes without foreground objects, given the fundamental application of object removal---where the desired outcome is a video without the object in question---and the standard reconstruction-based formulation of the problem~\cite{xu_deep_2019,chang_free-form_2019}, which assumes that the ground truth background appearance is known. Data from other video tasks, \eg, DAVIS~\cite{perazzi_benchmark_2016} and YouTube-VOS~\cite{xu_youtube-vos_2018}, do not satisfy this criterion since they generally feature foreground objects.

For these reasons, we collect our own videos of background-only scenes, similar to Zhang \etal~\cite{zhang_internal_2019}. In particular, we target scenic landscape videos in which people have filmed natural outdoor locations from both casual and cinematic viewpoints. Because the primary subject of these videos is the background, they are substantially less likely to contain prominent foreground objects, and are thus good targets for curating our source video collection.

To collect background scene videos, we first search Flickr~\cite{smugmug_inc_flickr_nodate} using the query term ``scenic'', and retain videos from a fixed set of users who have primarily uploaded high-quality, non-post-processed content between 2017-2019. Then, we apply a combination of automated and manual filtering to remove videos with foreground objects or shot transitions. Finally, we split the filtered videos into clips containing between 45-90 frames, yielding a total of 1,250 clips (examples are shown in Figure~\ref{fig:dataset-overview}). Our clips outnumber those of the DAVIS train/val set by a factor of ten. Additional details are provided in the supplementary materials.

\subsection{Annotating DEVIL Source Video Attributes}
\label{sec:annotating-devil-source-video}

For our DEVIL source videos, we annotate two types of content attributes: camera motion and BG scene motion (Figure~\ref{fig:dataset-overview}a). \textbf{Camera motion} encompasses frame-to-frame differences that are induced by changes in the camera's pose relative to the scene (\ie, camera extrinsics); \textbf{BG scene motion} refers to frame-to-frame differences that result from changes in the scene itself, such as running bodies of water or trees that sway due to strong winds (\ie, motion among ``stuff'' classes in the object detection sense~\cite{forsyth_finding_1996}).

We select these attributes for two reasons. First, they represent two sources of complex motion with different low-level characteristics that video inpainting models must replicate well to produce convincing predictions. Second, they impact video inpainting models by influencing the similarity and relevance of appearance information across frames. For instance, high camera motion can reveal or obscure parts of the scene, or otherwise change the scene's appearance due to perspective; high BG scene motion continuously changes the frame-wise appearance of textures.

These attributes are difficult to quantify concretely based on RGB video frames alone; however, it is possible to distinguish extreme examples of low and high motion by visual inspection and proxy estimates. Thus, for a given attribute, we label videos as containing either low or high motion, but only for a small percentage of videos lying at the extreme ends (videos not labeled for the given attribute may still appear in slices that do not control for it). Not only does this improve label accuracy, it also magnifies any performance differences caused by changing a given attribute between low and high settings, thereby highlighting failure modes.

To annotate camera motion, we use classical affine alignment techniques and measure the amount of invalid pixels introduced via warping as a proxy for camera motion; we then threshold the result on either side to produce low and high motion labels. As for BG scene motion, we manually assign low and high labels based on the percentage of the field of view that contains large running bodies of water. Further details can be found in the supplementary materials.

\subsection{DEVIL Masks and Attributes}
\label{sec:devil-masks-attributes}

For occlusion masks, we consider three attributes that influence the availability of relevant appearance information in nearby frames (Figure~\ref{fig:dataset-overview}a):
%
\begin{itemize}
  \item \textbf{FG displacement:} How much the mask's centroid moves over time with respect to the field of view;
  \item \textbf{FG pose motion:} How much the shape of the mask changes over time with respect to the field of view (independent of the displacement of its centroid); and
  \item \textbf{FG size:} The average number of pixels that are occupied by the mask per frame.
\end{itemize}
%
Masks with high FG displacement or pose motion reveal complementary parts of the scene over time, whereas FG size explicitly determines how much appearance information can be relied on as ground truth.

To generate masks with low and high settings for these attributes, we adapt the procedural blob generation strategy by Chang \etal~\cite{chang_free-form_2019}. In particular, we adjust their stroke width, velocity, and stochasticity parameters to correspond to low or high FG displacement, pose motion, and size. Further details are available in the supplementary materials.

\section{The DEVIL Evaluation}
\label{sec:devil-evaluation}

\subsection{Slices of the DEVIL Dataset}

The na\"ive way to evaluate on the DEVIL dataset would be to randomly sample a test set of paired source videos and occlusion masks without accounting for their attributes; however, this provides little insight into the failure modes that cause prediction errors for a given method. Instead, we control for one attribute at a time to isolate its impact on the prediction. Specifically, for each attribute setting, we construct \textit{slices} of the DEVIL dataset, \ie, pre-determined sets of video-mask pairs where the given attribute is fixed as low or high and the others are uncontrolled. By reporting performance on each slice separately, our benchmark can methodically highlight failure modes in a \textit{quantitative} manner that is \textit{comparable across methods}, which has not been considered in prior work.

We construct the DEVIL dataset slices as follows. Given the desired attribute setting (\eg, low camera motion), we randomly sample either 150 source videos or masks with that setting (recall that an attribute applies exclusively to either the source video or the mask modality). Then, within the other modality, we sample 150 instances from all available DEVIL instances (\eg, for the low camera motion slice, we sample all rendered DEVIL masks). Finally, we pair together the selected source videos and masks.

\subsection{Evaluation Metrics}
\label{sec:evaluation-metrics}

\begin{figure}
  \centering
  \begin{subfigure}{0.3\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/gt/frame_0005_gt}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/gt/frame_0006_gt}
    \end{subfigure}
    \caption{Ground truth}
  \end{subfigure}
  \hspace{1pt}
  \begin{subfigure}{0.3\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/vinet/frame_0005_pred.pdf}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/vinet/frame_0006_pred}
    \end{subfigure}
    \caption{VINet}
  \end{subfigure}
  \hspace{1pt}
  \begin{subfigure}{0.3\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/cpnet/frame_0005_pred}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/blurry/cpnet/frame_0006_pred}
    \end{subfigure}
    \caption{CPNet}
  \end{subfigure}
  \caption{High temporal consistency may indicate overly blurry predictions if reconstruction or realism performance is low (as shown in the results of VINet and CPNet). The area to be inpainted is outlined in yellow in (a).}
  \label{fig:blurry}
  \vspace{-10pt}
\end{figure}

We evaluate on composited inpainting results (\ie, the known region is composited over the inpainting prediction). Inputs are resized to 832$\times$480 resolution; for methods that cannot consume this resolution, we apply mirror padding to both the source video and the mask, run the method, and crop out padded regions from the result for fairness. We quantify performance along three axes of inpainting quality---reconstruction, realism, and temporal consistency---as described in the remainder of this section.

\paragraphheader{Reconstruction} captures the extent to which a video inpainting method predicts the original content in a given reference video (\ie, the version of the video without the occlusion mask). We report two reconstruction metrics: the Learned Perceptual Image Patch Similarity (LPIPS) metric~\cite{zhang_unreasonable_2018} with a pre-trained AlexNet backbone~\cite{krizhevsky_imagenet_2012}, and our own video-based variant called the Perceptual Video Clip Similarity (PVCS) metric with a pre-trained I3D backbone~\cite{carreira_quo_2017}. These metrics measure the distance between corresponding features of a deep neural network. LPIPS is computed between corresponding frames of the reference and inpainted video, whereas PVCS is computed between corresponding 10-frame clips in a sliding window.

\paragraphheader{Realism} indicates how well the inpainting result resembles the appearance and motion observed in a reference set of real videos, independent of the original video from which the input is derived. Unlike reconstruction, realism enforces a smaller penalty for deviating from the original content as long as the prediction exhibits sensible appearance and motion.
For our image-based realism metric, we use the Fr\'echet Inception Distance~\cite{heusel_gans_2017} (FID), which fits multivariate normal distributions over the feature activations of two sets of images and measures their distance; in our case, the two sets correspond to all predicted frames and all reference frames. We also report the video-based equivalent Video FID~\cite{kim_deep_2019} (VFID), which corresponds to the sets of all inpainted videos and all reference videos (the features are extracted from a pre-trained I3D backbone~\cite{carreira_quo_2017}).

\paragraphheader{Temporal consistency} measures the proliferation of flickering artifacts, \ie, how much colors at corresponding points of the scene change between consecutive frames. We adapt the patch consistency metric, denoted PCons, from Gupta \etal~\cite{gupta_characterizing_2017}: for each frame, we extract the 50$\times$50 patch at the centroid of the occlusion mask, compute the maximum Peak Signal-to-Noise Ratio (PSNR) between this patch and neighboring patches in the next frame, and average the result across all frames. Note that stronger temporal consistency is not always ideal: low-quality predictions, such as constant-color or blurry inpainting results, can produce high temporal consistency scores (see Figure~\ref{fig:blurry}).

\section{Experiments}
\label{sec:experiments}

\begin{figure*}
  \begin{subfigure}[b]{0.72\linewidth}
    \includegraphics[width=\linewidth]{figs/absolute-performance}
    \stepcounter{table}
    \caption*{Table \thetable: The performance of each inpainting method on each DEVIL slice and evaluation metric. Bold indicates the best method; \downtriangle{} and \uptriangle{} indicate that lower or higher is better, respectively.}
    \label{tab:absolute-performance}
  \end{subfigure}
  \hfill
  \begin{subfigure}[b]{0.25\linewidth}
    \begin{subfigure}{0.98\linewidth}
      \includegraphics[trim=0px 30px 0px 30px,clip,width=\linewidth]{figs/model-performance/lpips}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
      \includegraphics[trim=0px 30px 0px 30px,clip,width=\linewidth]{figs/model-performance/pvcs}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
      \includegraphics[trim=0px 30px 0px 30px,clip,width=\linewidth]{figs/model-performance/fid}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
      \includegraphics[trim=0px 30px 0px 30px,clip,width=\linewidth]{figs/model-performance/vfid}
    \end{subfigure}
    \begin{subfigure}{0.98\linewidth}
      \includegraphics[trim=0px 30px 0px 30px,clip,width=\linewidth]{figs/model-performance/pcons}
    \end{subfigure}
    \caption*{Figure \thefigure: Mean performance of each method across all DEVIL slices. Error bars show standard error across the ten slices.}
    \label{fig:model-performance}
  \end{subfigure}
  \vspace{-4pt}
\end{figure*}

To demonstrate the utility of our DEVIL benchmark, we analyze the performance of seven representative state-of-the-art video inpainting methods, using the publicly-available code, model weights, and default runtime arguments provided by the original authors:
%
\begin{itemize}
  \item \textbf{Joint optimization of flow and color (JointOpt)~\cite{huang_temporally_2016}:} Alternates between optimizing an optical flow estimate and finding suitable patches along the flow.
  \item \textbf{VINet~\cite{kim_deep_2019}:} Recurrently predicts the next frame by warping intermediate features spatially via optical flow.
  \item \textbf{Deep Flow Completion Network (DFCNet)~\cite{xu_deep_2019}:} Predicts the optical flow of the video, then inpaints the missing region by propagating known values along the flow.
  \item \textbf{Copy-Paste Network (CPNet)~\cite{lee_copy-and-paste_2019}:} Estimates affine transformations between frames via a task-driven DNN, then copies features across aligned frames via attention.
  \item \textbf{Onion Peel Network (OPN)~\cite{oh_onion-peel_2019}:} Iteratively inpaints the exterior of the current missing region by attending to relevant locations in the known region.
  \item \textbf{Spatio-Temporal Transformer Network (STTN)~\cite{zeng_learning_2020}:} Decodes the missing region with a Transformer~\cite{vaswani_attention_2017} that consumes multi-scale patches from the entire video.
  \item \textbf{Flow-Edge Guided Video Completion (FGVC)~\cite{gao_flow-edge_2020}:} Extends DFCNet~\cite{xu_deep_2019} by leveraging flow between non-adjacent frames and using edge information to solve for piecewise-smooth flow predictions.
\end{itemize}

\subsection{Aggregate Analysis}

In Table~\hyperref[tab:absolute-performance]{1}, we report the performance of all evaluated methods on each DEVIL slice; in Figure~\hyperref[fig:model-performance]{3}, we compare their performance averaged across all slices. We observe that JointOpt, DFCNet, and FGVC consistently outrank or perform within one standard error of the other methods in terms of the reconstruction metrics LPIPS/PVCS and the realism metrics FID/VFID. They all explicitly solve for the optical flow of the inpainted video during inference, suggesting that \textit{computing task-driven flow is an essential ingredient in producing the highest-quality video inpainting results}. Additionally, JointOpt remains competitive among recent deep learning-based solutions, suggesting that improvements may arise by adapting traditional subroutines, \eg, PatchMatch~\cite{barnes_patchmatch_2009}, to deep learning.

The three mid-tier methods---OPN, STTN, and CPNet---borrow intermediate features across distant time steps, but do not use time as an ordered structure. Meanwhile, VINet models time through a recurrent unit, but has the shortest temporal receptive field among the evaluated methods and cannot propagate information from future time steps back through the entire video. These results indicate that \textit{modeling time as a proper ordered structure with long-range dependencies greatly improves inpainting quality.}

In terms of temporal consistency, DFCNet achieves the highest PCons since it propagates pixel values directly along the predicted flow maps of adjacent frames. Interestingly, JointOpt and FGVC achieve lower PCons despite also propagating values along the flow, likely due to their ability to transfer candidate values from non-adjacent frames. VINet and CPNet achieve high temporal consistency at the cost of low-quality predictions lacking appropriate texture or motion (Figure~\ref{fig:blurry}); the behaviors of these two models indicate that temporal consistency is most meaningful when reconstruction and realism performance is also high.

\begin{figure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/slice-difficulty/legend}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[trim=0px 20px 0px 0px,clip,width=0.9\linewidth]{figs/slice-difficulty/pvcs}
  \end{subfigure}
  \caption{Comparison of DEVIL slice difficulty based on average model performance (lower is better; error bars show standard error across the seven models). The type of content given at test time, especially the mask content, greatly affects the difficulty of the task.}
  \label{fig:slice-difficulty}
\end{figure}

\begin{table}
  \centering
  \includegraphics[width=0.75\linewidth]{figs/rank/rank}
  \caption{Methods sorted by performance from best to worst based on three variables: the metric (LPIPS/VFID), the \mbox{attribute} (FG displacement/camera motion), and the setting of said attribute (low/high). The strongest method (highlighted in bold) depends on all three variables, showing that no one method dominates our challenging benchmark.}
  \vspace{-12pt}
  \label{fig:rank}
\end{table}

\paragraphheader{DEVIL Attribute Difficulty} We now analyze how DEVIL attributes impact overall inpainting difficulty to highlight their utility in video inpainting evaluation. In Figure~\ref{fig:slice-difficulty}, we compare the difficulty of each DEVIL attribute setting by computing the average PVCS over all methods on the corresponding test slice. The overall impact of camera and BG scene motion is small due to the differing sensitivities of each method to these attributes (Section~\ref{sec:model-sensitivity-devil-attributes}); we observe similar trends under the other reconstruction and realism metrics (refer to the supplementary materials for details). In contrast, the mask attributes substantially impact the difficulty of video inpainting; specifically, higher FG displacement and pose motion, as well as smaller FG size, lead to better performance. Although this result is intuitive---more relevant appearance information is available in other frames when the occlusion mask is smaller and moves more over time---our work is the first to present quantitative evidence of these trends across a wide range of methods.

\subsection{Model Sensitivity to DEVIL Attributes}
\label{sec:model-sensitivity-devil-attributes}

\begin{figure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.86\linewidth]{figs/relative-difference/legend-video}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/relative-difference/cm}
  \end{subfigure}
  \caption{Relative improvement of each method under reconstruction and realism metrics when camera motion changes from low to high.}
  \label{fig:relative-difference-cm}
  \vspace{-1pt}
\end{figure}

\begin{figure}
  \centering
  \begin{subfigure}{0.38\linewidth}
    \centering
    \begin{subfigure}{0.95\linewidth}
      \includegraphics[width=\linewidth]{figs/vinet-cm/cm-l/vinet/frame_0000_pred}
    \end{subfigure}
    \begin{subfigure}{0.95\linewidth}
      \includegraphics[width=\linewidth]{figs/vinet-cm/cm-l/vinet/frame_0045_pred}
    \end{subfigure}
    \caption{Low camera motion}
  \end{subfigure}
  \begin{subfigure}{0.38\linewidth}
    \centering
    \begin{subfigure}{0.95\linewidth}
      \includegraphics[width=\linewidth]{figs/vinet-cm/cm-h/vinet/frame_0000_pred}
    \end{subfigure}
    \begin{subfigure}{0.95\linewidth}
      \includegraphics[width=\linewidth]{figs/vinet-cm/cm-h/vinet/frame_0020_pred}
    \end{subfigure}
    \caption{High camera motion}
  \end{subfigure}
  \caption{VINet prediction examples. VINet improves with high camera motion since content ``moves into'' the missing region (arrows show the direction of camera motion).}
  \label{fig:vinet-cm}
  \vspace{-12pt}
\end{figure}

Next, we compare the performance of each method on individual DEVIL slices to demonstrate the impact of video and mask content, as well as the metric, on their rankings. Table~\ref{fig:rank} lists the methods sorted by performance and grouped by three variables: (i) the metric, (ii) the DEVIL attribute, and (iii) the particular setting of the attribute (\ie, low or high). Note that the two attributes shown, FG displacement and camera motion, span the two modalities of the DEVIL dataset (masks and videos, respectively); also note that these three variables span the complexity of the DEVIL evaluation scheme in terms of metrics and dataset slices. Even among the eight different combinations of variables shown out of the possible 50, four methods achieve the best performance for at least one combination; this demonstrates that \emph{our DEVIL benchmark promotes substantial competition between video inpainting methods.}

Finally, we analyze the sensitivity of the methods to each DEVIL attribute by changing the label and plotting the relative difference in performance. Specifically, for a given attribute, we compute the relative improvement as $(\textrm{score}_\textrm{hi} - \textrm{score}_\textrm{lo}) / \textrm{score}_\textrm{lo}$ (or the negation of this value if a lower score is better), where $\textrm{score}_\textrm{hi}$ and $\textrm{score}_\textrm{lo}$ correspond to model performance on the high and low slices of the attribute, respectively. As evidenced by the following observations, our DEVIL attributes enable a fine-grained comparison of failure modes among different inpainting models.

In Figure~\ref{fig:relative-difference-cm}, we see divergent behavior among the methods when camera motion is increased: for example, STTN and CPNet experience dramatic performance drops under all reconstruction and realism metrics, whereas VINet experiences substantial gains. From a design standpoint, the behaviors of STTN and CPNet make sense because they rely on aligning patches or entire frames from other time steps to borrow their features, which can fail catastrophically under heavy camera motion. On the opposite end, VINet's behavior reflects its tendency to inpaint realistic textures only after they move into the missing region (Figure~\ref{fig:vinet-cm}), which is unlikely to occur without camera motion. Although these weaknesses can be found through visual inspection, DEVIL quantifies performance on representative slices to illuminate them more quickly and in a comparable manner.

\begin{figure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.86\linewidth]{figs/relative-difference/legend-video}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.9\linewidth]{figs/relative-difference/bsm}
  \end{subfigure}
  \caption{Relative improvement of each method under reconstruction and realism metrics when BG scene motion changes from low to high.}
  \label{fig:relative-difference-bsm}
\end{figure}

\begin{figure}
  \centering
  \begin{subfigure}{0.24\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/gt/frame_0000_gt}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/gt/frame_0005_gt}
    \end{subfigure}
    \caption{GT}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/dfcnet/frame_0000_pred}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/dfcnet/frame_0005_pred}
    \end{subfigure}
    \caption{DFCNet}
  \end{subfigure}
  \begin{subfigure}{0.24\linewidth}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/fgvc/frame_0000_pred}
    \end{subfigure}
    \begin{subfigure}{\linewidth}
      \includegraphics[width=\linewidth]{figs/alt-reality/fgvc/frame_0005_pred}
    \end{subfigure}
    \caption{FGVC}
  \end{subfigure}
  \caption{Inpainting predictions for high BG scene motion. DFCNet and FGVC predictions diverge from the original content, but still exhibit semantically sensible appearance.}
  \label{fig:alt-reality}
  \vspace{-12pt}
\end{figure}

\begin{figure}
  \begin{subfigure}{\linewidth}
    \centering
    \includegraphics[width=0.95\linewidth]{figs/relative-difference/legend-mask}
  \end{subfigure}
  \begin{subfigure}{\linewidth}
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{figs/relative-difference/fgd}
      \caption{FG displacement}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{figs/relative-difference/fgm}
      \caption{FG pose motion}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.32\linewidth}
      \includegraphics[width=\linewidth]{figs/relative-difference/fgs}
      \caption{FG size}
      \label{fig:relative-difference-mask-fgs}
    \end{subfigure}
  \end{subfigure}
  \caption{Relative improvement of each method under PVCS when mask attributes change from low to high.}
  \vspace{-10pt}
  \label{fig:relative-difference-mask}
\end{figure}

From Figure~\ref{fig:relative-difference-bsm}, we see that reconstruction performance under LPIPS and PVCS consistently worsens when BG scene motion increases, reflecting the challenge of replicating complex dynamics precisely. Interestingly, frame realism under FID actually improves dramatically for some methods such as DFCNet and FGVC because they inpaint ``alternate realities'', \ie, appearance that diverges from the original content, but still captures the original broad structure (Figure~\ref{fig:alt-reality}). Among the methods that explicitly infer and propagate across flow (FGVC, JointOpt, and DFCNet), only JointOpt achieves worse frame realism performance, suggesting that \textit{video inpainting quality can be improved by simply learning flow in a task-driven, end-to-end manner.}

Moving on to mask attributes, we show in Figure~\ref{fig:relative-difference-mask}a-b that all methods perform better with increased FG displacement and pose motion, indicating that they all leverage the increased availability of background information. The flow propagation methods generally benefit the most, likely due to the explicit transmission of more ground-truth appearance information along predicted flows. We observe similar trends under the other reconstruction and realism metrics (details are available in the supplementary materials).

In Figure~\ref{fig:relative-difference-mask-fgs}, we observe worse performance when the mask FG size grows, reflecting the inherently greater difficulty of inpainting more values. Although this trend is universal and intuitive, the quantitative difference between methods still lends insight into their failure modes. For example, OPN is most sensitive to the increased mask size because it must iteratively inpaint more outer layers of the unknown region based on its own predictions, thereby accumulating error across more iterations.

\section{Conclusion}

We have presented the DEVIL benchmark for video inpainting and used it to analyze seven state-of-the-art methods, thereby providing the largest fine-grained analysis of video inpainting to our knowledge. By controlling for five content attributes of the source videos and masks used at test time, our analyses have provided novel insight into the behaviors, strengths, and weaknesses of these methods.

Upon publication, we plan to open-source our benchmark data and tools to foster the community's adoption of diagnostic video inpainting evaluation. In future work, we plan to analyze the impact of even more content attributes on inpainting performance, including those pertaining to foreground objects in the source video.

